How Far Have We Gone in Binary Code Understanding Using Large Language Models

Binary code analysis plays a pivotal role in various software security applications, such as software maintenance, malware detection, software vulnerability discovery, patch analysis, etc. However, unlike source code, understanding binary code is challenging for reverse engineers due to the absence of semantic information. Therefore, automated tools are needed to assist human players in interpreting binary code. In recent years, two groups of technologies have shown promising prospects: (1) Deep learning-based technologies have demonstrated competitive results in tasks related to binary code understanding, furthermore, (2) Large Language Models (LLMs) have been extensively pre-trained at the source-code level for tasks such as code understanding and generation. This makes participants wonder about the ability of LLMs in binary code understanding. In this work, we propose a benchmark to evaluate the effectiveness of LLMs in real-world reverse engineering scenarios. The benchmark covers two key binary code understanding tasks, including function name recovery and binary code summarization. We gain valuable insights into their capabilities and limitations through extensive evaluations of popular LLMs using our benchmark. Our evaluations reveal that existing LLMs can understand binary code to a certain extent, thereby improving the efficiency of binary code analysis. Our results highlight the great potential of the LLMs in advancing the field of binary code understanding.

==> ref.tex <==

@inproceedings{Chen2023pst,
      author={Chen, Guoqiang and Gao, Han and Zhang, Jie and He, Yanru and Cheng, Shaoyin and Zhang, Weiming},
      booktitle={2023 20th Annual International Conference on Privacy, Security and Trust (PST)}, 
      title={Investigating Neural-based Function Name Reassignment from the Perspective of Binary Code Representation}, 
      year={2023},
      volume={},
      number={},
      pages={1-11},
      doi={10.1109/PST58708.2023.10320193}
}

@inproceedings{Xiong2023ase,
      author={Xiong, Jiaqi and Chen, Guoqiang and Chen, Kejiang and Gao, Han and Cheng, Shaoyin and Zhang, Weiming},
      booktitle={2023 38th IEEE/ACM International Conference on Automated Software Engineering (ASE)}, 
      title={HexT5: Unified Pre-Training for Stripped Binary Code Information Inference}, 
      year={2023},
      volume={},
      number={},
      pages={774-786},
      doi={10.1109/ASE56229.2023.00099}
}

@inproceedings{nfre2021issta,
    author = {Gao, Han and Cheng, Shaoyin and Xue, Yinxing and Zhang, Weiming},
    title = {A Lightweight Framework for Function Name Reassignment Based on Large-Scale Stripped Binaries},
    year = {2021},
    isbn = {9781450384599},
    publisher = {Association for Computing Machinery},
    address = {New York, NY, USA},
    url = {https://doi.org/10.1145/3460319.3464804},
    doi = {10.1145/3460319.3464804},
    booktitle = {Proceedings of the 30th ACM SIGSOFT International Symposium on Software Testing and Analysis},
    pages = {607–619},
    numpages = {13},
    keywords = {Reverse Engineering, Neural Networks, Binary Analysis},
    location = {Virtual, Denmark},
    series = {ISSTA 2021}
}

@inproceedings{bint52023saner,
      author={Al-Kaswan, Ali and Ahmed, Toufique and Izadi, Maliheh and Sawant, Anand Ashok and Devanbu, Premkumar and van Deursen, Arie},
      booktitle={2023 IEEE International Conference on Software Analysis, Evolution and Reengineering (SANER)}, 
      title={Extending Source Code Pre-Trained Language Models to Summarise Decompiled Binaries}, 
      year={2023},
      volume={},
      number={},
      pages={260-271},
      doi={10.1109/SANER56733.2023.00033}
}

@article{nero2020,
    author = {David, Yaniv and Alon, Uri and Yahav, Eran},
    title = {Neural Reverse Engineering of Stripped Binaries Using Augmented Control Flow Graphs},
    year = {2020},
    issue_date = {November 2020},
    publisher = {Association for Computing Machinery},
    address = {New York, NY, USA},
    volume = {4},
    number = {OOPSLA},
    url = {https://doi.org/10.1145/3428293},
    doi = {10.1145/3428293},
    journal = {Proc. ACM Program. Lang.},
    month = {nov},
    articleno = {225},
    numpages = {28},
    keywords = {Neural Reverse Engineering, Static Binary Analysis}
    }

@inproceedings{symlm2022ccs,
    author = {Jin, Xin and Pei, Kexin and Won, Jun Yeon and Lin, Zhiqiang},
    title = {SymLM: Predicting Function Names in Stripped Binaries via Context-Sensitive Execution-Aware Code Embeddings},
    year = {2022},
    isbn = {9781450394505},
    publisher = {Association for Computing Machinery},
    address = {New York, NY, USA},
    url = {https://doi.org/10.1145/3548606.3560612},
    doi = {10.1145/3548606.3560612},
    booktitle = {Proceedings of the 2022 ACM SIGSAC Conference on Computer and Communications Security},
    pages = {1631–1645},
    numpages = {15},
    keywords = {function name prediction, calling context, transfer learning, binary reverse engineering, execution behavior},
    location = {Los Angeles, CA, USA},
    series = {CCS '22}
    }

@article{Canfora2011,
    author = {Canfora, Gerardo and Di Penta, Massimiliano and Cerulo, Luigi},
    title = {Achievements and Challenges in Software Reverse Engineering},
    year = {2011},
    issue_date = {April 2011},
    publisher = {Association for Computing Machinery},
    address = {New York, NY, USA},
    volume = {54},
    number = {4},
    issn = {0001-0782},
    url = {https://doi.org/10.1145/1924421.1924451},
    doi = {10.1145/1924421.1924451},
    journal = {Commun. ACM},
    month = {apr},
    pages = {142–151},
    numpages = {10}
    }

@article{Alrabaee2022,
author = {Alrabaee, Saed and Debbabi, Mourad and Wang, Lingyu},
title = {A Survey of Binary Code Fingerprinting Approaches: Taxonomy, Methodologies, and Features},
year = {2022},
issue_date = {January 2023},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
volume = {55},
number = {1},
issn = {0360-0300},
url = {https://doi.org/10.1145/3486860},
doi = {10.1145/3486860},
journal = {ACM Comput. Surv.},
month = {jan},
articleno = {19},
numpages = {41},
keywords = {reverse engineering, software security, Binary code analysis}
}

@Misc{Ghidra,
howpublished = {\url{https://github.com/NationalSecurityAgency/ghidra}},
year = {2023},
title = {"Ghidra"},
author = {NationalSecurityAgency}
}

@Misc{IDA,
howpublished = {\url{https://www.hex-rays.com/products/ ida}},
year = {2023},
title = {"IDA Pro"},
author = {Hex-RaysSA}
}

@Misc{BinaryNinja,
howpublished = {\url{https://binary.ninja/}},
year = {2023},
title = {"Binary Ninja"},
author = {Vector35}
}

@inproceedings{Meng2016issta,
author = {Meng, Xiaozhu and Miller, Barton P.},
title = {Binary Code is Not Easy},
year = {2016},
isbn = {9781450343909},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/2931037.2931047},
doi = {10.1145/2931037.2931047},
booktitle = {Proceedings of the 25th International Symposium on Software Testing and Analysis},
pages = {24–35},
numpages = {12},
keywords = {Challenging code constructs, Jump table model, Static binary code analysis},
location = {Saarbr\"{u}cken, Germany},
series = {ISSTA 2016}
}

@techreport{Gellenbeck1991,
author = {Gellenbeck, Edward M. and Cook, Curtis R.},
title = {An Investigation of Procedure and Variable Names as Beacons During Program Comprehension},
year = {1991},
publisher = {Oregon State University},
address = {USA}
}

@inproceedings{Sridhara2010ase,
author = {Sridhara, Giriprasad and Hill, Emily and Muppaneni, Divya and Pollock, Lori and Vijay-Shanker, K.},
title = {Towards Automatically Generating Summary Comments for Java Methods},
year = {2010},
isbn = {9781450301169},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/1858996.1859006},
doi = {10.1145/1858996.1859006},
booktitle = {Proceedings of the 25th IEEE/ACM International Conference on Automated Software Engineering},
pages = {43–52},
numpages = {10},
keywords = {natural language program analysis, method summarization, comment generation},
location = {Antwerp, Belgium},
series = {ASE '10}
}

@inproceedings{wang-etal-2021-codet5,
    title = "{C}ode{T}5: Identifier-aware Unified Pre-trained Encoder-Decoder Models for Code Understanding and Generation",
    author = "Wang, Yue  and
      Wang, Weishi  and
      Joty, Shafiq  and
      Hoi, Steven C.H.",
    booktitle = "Proceedings of the 2021 Conference on Empirical Methods in Natural Language Processing",
    month = "nov",
    year = "2021",
    address = "Online and Punta Cana, Dominican Republic",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/2021.emnlp-main.685",
    doi = "10.18653/v1/2021.emnlp-main.685",
    pages = "8696--8708"
}

@misc{codellama2023rozière,
      title={Code Llama: Open Foundation Models for Code}, 
      author={Baptiste Rozière and Jonas Gehring and Fabian Gloeckle and Sten Sootla and Itai Gat and Xiaoqing Ellen Tan and Yossi Adi and Jingyu Liu et.al.},
      year={2023},
      eprint={2308.12950},
      archivePrefix={arXiv},
      primaryClass={cs.CL}
}

@misc{wizardcoder2023luo,
      title={WizardCoder: Empowering Code Large Language Models with Evol-Instruct}, 
      author={Ziyang Luo and Can Xu and Pu Zhao and Qingfeng Sun and Xiubo Geng and Wenxiang Hu and Chongyang Tao and Jing Ma and Qingwei Lin and Daxin Jiang},
      year={2023},
      eprint={2306.08568},
      archivePrefix={arXiv},
      primaryClass={cs.CL}
}

@misc{vicuna2023judging,
      title={Judging LLM-as-a-Judge with MT-Bench and Chatbot Arena}, 
      author={Lianmin Zheng and Wei-Lin Chiang and Ying Sheng and Siyuan Zhuang and Zhanghao Wu and Yonghao Zhuang and Zi Lin and Zhuohan Li and Dacheng Li and Eric. P Xing and Hao Zhang and Joseph E. Gonzalez and Ion Stoica},
      year={2023},
      eprint={2306.05685},
      archivePrefix={arXiv},
      primaryClass={cs.CL}
}

@misc{chatgpt2022training,
      title={Training language models to follow instructions with human feedback}, 
      author={Long Ouyang and Jeff Wu and Xu Jiang and Diogo Almeida and Carroll L. Wainwright and Pamela Mishkin and Chong Zhang et.al.},
      year={2022},
      eprint={2203.02155},
      archivePrefix={arXiv},
      primaryClass={cs.CL}
}

@misc{chatglm2023glm130b,
      title={GLM-130B: An Open Bilingual Pre-trained Model}, 
      author={Aohan Zeng and Xiao Liu and Zhengxiao Du and Zihan Wang and Hanyu Lai and Ming Ding and Zhuoyi Yang et.al.},
      year={2023},
      eprint={2210.02414},
      archivePrefix={arXiv},
      primaryClass={cs.CL}
}

@misc{codegen2_2023nijkamp,
      title={CodeGen2: Lessons for Training LLMs on Programming and Natural Languages}, 
      author={Erik Nijkamp and Hiroaki Hayashi and Caiming Xiong and Silvio Savarese and Yingbo Zhou},
      year={2023},
      eprint={2305.02309},
      archivePrefix={arXiv},
      primaryClass={cs.LG}
}

@misc{Llama2023llama,
      title={Llama 2: Open Foundation and Fine-Tuned Chat Models}, 
      author={Hugo Touvron and Louis Martin and Kevin Stone and Peter Albert and Amjad Almahairi and Yasmine Babaei et.al.},
      year={2023},
      eprint={2307.09288},
      archivePrefix={arXiv},
      primaryClass={cs.CL}
}

@article{David2020Neural,
author = {David, Yaniv and Alon, Uri and Yahav, Eran},
title = {Neural Reverse Engineering of Stripped Binaries Using Augmented Control Flow Graphs},
year = {2020},
issue_date = {November 2020},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
volume = {4},
number = {OOPSLA},
url = {https://doi.org/10.1145/3428293},
doi = {10.1145/3428293},
journal = {Proc. ACM Program. Lang.},
month = {nov},
articleno = {225},
numpages = {28},
keywords = {Neural Reverse Engineering, Static Binary Analysis}
}

@inproceedings{papineni-etal-2002-bleu,
    title = "{B}leu: a Method for Automatic Evaluation of Machine Translation",
    author = "Papineni, Kishore  and
      Roukos, Salim  and
      Ward, Todd  and
      Zhu, Wei-Jing",
    booktitle = "Proceedings of the 40th Annual Meeting of the Association for Computational Linguistics",
    year = "2002",
    address = "Philadelphia, Pennsylvania, USA",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/P02-1040",
    doi = "10.3115/1073083.1073135",
    pages = "311--318",
}

@inproceedings{lin-2004-rouge,
    title = "{ROUGE}: A Package for Automatic Evaluation of Summaries",
    author = "Lin, Chin-Yew",
    booktitle = "Text Summarization Branches Out",
    year = "2004",
    address = "Barcelona, Spain",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/W04-1013",
    pages = "74--81",
}

@article{meteor2009Lavie,
author = {Lavie, Alon and Denkowski, Michael J.},
title = {The Meteor Metric for Automatic Evaluation of Machine Translation},
year = {2009},
issue_date = {September 2009},
publisher = {Kluwer Academic Publishers},
address = {USA},
volume = {23},
number = {2–3},
issn = {0922-6567},
url = {https://doi.org/10.1007/s10590-009-9059-4},
doi = {10.1007/s10590-009-9059-4},
journal = {Machine Translation},
month = {sep},
pages = {105–115},
numpages = {11},
keywords = {MT Evaluation, Machine translation, Automatic metrics}
}

@ARTICLE{Kim2023tse,
  author={Kim, Dongkwan and Kim, Eunsoo and Cha, Sang Kil and Son, Sooel and Kim, Yongdae},
  journal={IEEE Transactions on Software Engineering}, 
  title={Revisiting Binary Code Similarity Analysis Using Interpretable Feature Engineering and Lessons Learned}, 
  year={2023},
  volume={49},
  number={4},
  pages={1661-1682},
  doi={10.1109/TSE.2022.3187689}}

@inproceedings{Duan2020DeepBinDiff,
author = {Duan, Yue and Li, Xuezixiang and Wang, Jinghan and Yin, Heng},
year = {2020},
month = {01},
pages = {},
title = {DeepBinDiff: Learning Program-Wide Code Representations for Binary Diffing},
doi = {10.14722/ndss.2020.24311}
}

@inproceedings{Pei2021state,
author = {Pei, Kexin and Guan, Jonas and Broughton, Matthew and Chen, Zhongtian and Yao, Songchen and Williams-King, David and Ummadisetty, Vikas and Yang, Junfeng and Ray, Baishakhi and Jana, Suman},
title = {StateFormer: Fine-Grained Type Recovery from Binaries Using Generative State Modeling},
year = {2021},
isbn = {9781450385626},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/3468264.3468607},
doi = {10.1145/3468264.3468607},
booktitle = {Proceedings of the 29th ACM Joint Meeting on European Software Engineering Conference and Symposium on the Foundations of Software Engineering},
pages = {690–702},
numpages = {13},
keywords = {Machine Learning for Program Analysis, Type Inference, Transfer Learning, Reverse Engineering},
location = {Athens, Greece},
series = {ESEC/FSE 2021}
}

@inproceedings{Zhang2023lev,
author = {Zhang, Yifan},
title = {Leveraging Artificial Intelligence on Binary Code Comprehension},
year = {2023},
isbn = {9781450394758},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/3551349.3559564},
doi = {10.1145/3551349.3559564},
booktitle = {Proceedings of the 37th IEEE/ACM International Conference on Automated Software Engineering},
articleno = {125},
numpages = {3},
location = {Rochester, MI, USA},
series = {ASE '22}
}

@inproceedings{He2018debin,
author = {He, Jingxuan and Ivanov, Pesho and Tsankov, Petar and Raychev, Veselin and Vechev, Martin},
title = {Debin: Predicting Debug Information in Stripped Binaries},
year = {2018},
isbn = {9781450356930},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/3243734.3243866},
doi = {10.1145/3243734.3243866},
booktitle = {Proceedings of the 2018 ACM SIGSAC Conference on Computer and Communications Security},
pages = {1667–1680},
numpages = {14},
keywords = {debug information, binary code, security, machine learning},
location = {Toronto, Canada},
series = {CCS '18}
}

@misc{Dwarfformat,
    howpublished = {\url{https://dwarfstd.org/doc/DWARF4.pdf}},
    title={Dwarf debugging information format version 4}, 
    year = {2010},
    author = {I. UNIX International}
}

@INPROCEEDINGS{Maletic2015Exploration,
  author={Maletic, Jonathan I. and Collard, Michael L.},
  booktitle={2015 IEEE/ACM 37th IEEE International Conference on Software Engineering}, 
  title={Exploration, Analysis, and Manipulation of Source Code Using srcML}, 
  year={2015},
  volume={2},
  number={},
  pages={951-952},
  doi={10.1109/ICSE.2015.302}}

@misc{zhang2023sectests,
      title={How well does LLM generate security tests?}, 
      author={Ying Zhang and Wenjia Song and Zhengjie Ji and Danfeng and Yao and Na Meng},
      year={2023},
      eprint={2310.00710},
      archivePrefix={arXiv},
      primaryClass={cs.CR}
}

@inproceedings{HowEffective_ISSTA_2023,
    author = {Wu, Yi and Jiang, Nan and Pham, Hung Viet and Lutellier, Thibaud and Davis, Jordan and Tan, Lin and Babkin, Petr and Shah, Sameena},
    title = {How Effective Are Neural Networks for Fixing Security Vulnerabilities},
    year = {2023},
    isbn = {9798400702211},
    publisher = {Association for Computing Machinery},
    address = {New York, NY, USA},
    url = {https://doi.org/10.1145/3597926.3598135},
    doi = {10.1145/3597926.3598135},
    booktitle = {Proceedings of the 32nd ACM SIGSOFT International Symposium on Software Testing and Analysis},
    pages = {1282–1294},
    numpages = {13},
    keywords = {Vulnerability, Automated Program Repair, Language Model, AI and Software Engineering},
    location = {<conf-loc>, <city>Seattle</city>, <state>WA</state>, <country>USA</country>, </conf-loc>},
    series = {ISSTA 2023}
}

@inproceedings{Junod2015obf,
author = {Junod, Pascal and Rinaldini, Julien and Wehrli, Johan and Michielin, Julie},
title = {Obfuscator-LLVM -- Software Protection for the Masses},
year = {2015},
isbn = {9781467370943},
publisher = {IEEE Computer Society},
address = {USA},
url = {https://doi.org/10.1109/SPRO.2015.10},
doi = {10.1109/SPRO.2015.10},
booktitle = {Proceedings of the 2015 IEEE/ACM 1st International Workshop on Software Protection},
pages = {3–9},
numpages = {7},
series = {SPRO '15}
}

@misc{deepseekcoder,
      title={DeepSeek-Coder: When the Large Language Model Meets Programming -- The Rise of Code Intelligence}, 
      author={Daya Guo and Qihao Zhu and Dejian Yang and Zhenda Xie and Kai Dong and Wentao Zhang and Guanting Chen and Xiao Bi and Y. Wu and Y. K. Li and Fuli Luo and Yingfei Xiong and Wenfeng Liang},
      year={2024},
      eprint={2401.14196},
      archivePrefix={arXiv},
      primaryClass={cs.SE}
}

@misc{mixtral2024jiang,
      title={Mixtral of Experts}, 
      author={Albert Q. Jiang and Alexandre Sablayrolles and Antoine Roux and Arthur Mensch and Blanche Savary and Chris Bamford and Devendra Singh Chaplot and Diego de las Casas and Emma Bou Hanna and Florian Bressand and Gianna Lengyel and Guillaume Bour and Guillaume Lample and Lélio Renard Lavaud and Lucile Saulnier and Marie-Anne Lachaux and Pierre Stock and Sandeep Subramanian and Sophia Yang and Szymon Antoniak and Teven Le Scao and Théophile Gervet and Thibaut Lavril and Thomas Wang and Timothée Lacroix and William El Sayed},
      year={2024},
      eprint={2401.04088},
      archivePrefix={arXiv},
      primaryClass={cs.LG}
}

@inproceedings{Zhang2021sp,
  author={Zhang, Zhuo and You, Wei and Tao, Guanhong and Aafer, Yousra and Liu, Xuwei and Zhang, Xiangyu},
  booktitle={2021 IEEE Symposium on Security and Privacy (SP)}, 
  title={StochFuzz: Sound and Cost-effective Fuzzing of Stripped Binaries by Incremental and Stochastic Rewriting}, 
  year={2021},
  volume={},
  number={},
  pages={659-676},
  keywords={Privacy;Runtime;Instruments;Aggregates;Fuzzing;Probabilistic logic;Hardware;Binary-Rewriting;Fuzz},
  doi={10.1109/SP40001.2021.00109}}

@inproceedings{Giffin2004EfficientCI,
  title={Efficient Context-Sensitive Intrusion Detection},
  author={Jonathon T. Giffin and Somesh Jha and Barton P. Miller},
  booktitle={Network and Distributed System Security Symposium},
  year={2004},
}

@inproceedings{Patrick2020acsac,
author = {Patrick-Evans, James and Cavallaro, Lorenzo and Kinder, Johannes},
title = {Probabilistic Naming of Functions in Stripped Binaries},
year = {2020},
isbn = {9781450388580},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/3427228.3427265},
doi = {10.1145/3427228.3427265},
booktitle = {Proceedings of the 36th Annual Computer Security Applications Conference},
pages = {373–385},
numpages = {13},
keywords = {binaries, function names, machine learning},
location = {<conf-loc>, <city>Austin</city>, <country>USA</country>, </conf-loc>},
series = {ACSAC '20}
}

@misc{FFmpeg,
  author = {FFmpeg},
  year = {2024},
  url = {https://github.com/FFmpeg/FFmpeg},
}

@misc{Redis,
  author = {Redis},
  year = {2024},
  url = {https://github.com/redis/redis},
}

@misc{Curl,
  author = {Curl},
  year = {2024},
  url = {https://github.com/curl/curl},
}

@misc{Masscan,
  author = {Masscan},
  year = {2024},
  url = {https://github.com/robertdavidgraham/masscan},
}

@misc{Llama2.c,
  author = {Llama2.c},
  year = {2024},
  url = {https://github.com/karpathy/llama2.c},
}

@misc{whisper.cpp,
  author = {Whisper.cpp},
  year = {2024},
  url = {https://github.com/ggerganov/whisper.cpp},
}

@misc{OpenSSL,
  author = {OpenSSL},
  year = {2024},
  url = {https://github.com/openssl/openssl},
}

@misc{7z,
  author = {7z},
  year = {2024},
  url = {https://github.com/kornelski/7z},
}

@misc{zstd,
  author = {zstd},
  year = {2024},
  url = {https://github.com/facebook/zstd},
}

@misc{ImageMagick,
  author = {ImageMagick},
  year = {2024},
  url = {https://github.com/ImageMagick/ImageMagick},
}

@misc{Libvips,
  author = {Libvips},
  year = {2024},
  url = {https://github.com/libvips/libvips},
}

@misc{Libexpat,
  author = {Libexpat},
  year = {2024},
  url = {https://github.com/libexpat/libexpat},
}

@misc{Ultrajson,
  author = {Ultrajson},
  year = {2024},
  url = {https://github.com/ultrajson/ultrajson},
}

@misc{pei2021trex,
      title={Trex: Learning Execution Semantics from Micro-Traces for Binary Similarity}, 
      author={Kexin Pei and Zhou Xuan and Junfeng Yang and Suman Jana and Baishakhi Ray},
      year={2021},
      eprint={2012.08680},
      archivePrefix={arXiv},
      primaryClass={cs.CR}
}

@Misc{HuggingFace,
  author = {HuggingFace},
  year = {2024},
  url = {https://huggingface.co/}
}

@Misc{PyTorch,
    author = {PyTorch},
    url = {https://pytorch.org/},
    year = {2024},
}

@Misc{Transformers,
    author = {Transformers},
    url = {https://huggingface.co/},
    year = {2024},
}

@Misc{DeepSpeed,
    author = {DeepSpeed},
    url = {https://www.deepspeed.ai/},
    year = {2024},
}

@misc{feng2020codebert,
      title={CodeBERT: A Pre-Trained Model for Programming and Natural Languages}, 
      author={Zhangyin Feng and Daya Guo and Duyu Tang and Nan Duan and Xiaocheng Feng and Ming Gong and Linjun Shou and Bing Qin and Ting Liu and Daxin Jiang and Ming Zhou},
      year={2020},
      eprint={2002.08155},
      archivePrefix={arXiv},
      primaryClass={cs.CL}
}

@misc{fried2023incoder,
      title={InCoder: A Generative Model for Code Infilling and Synthesis}, 
      author={Daniel Fried and Armen Aghajanyan and Jessy Lin and Sida Wang and Eric Wallace and Freda Shi and Ruiqi Zhong and Wen-tau Yih and Luke Zettlemoyer and Mike Lewis},
      year={2023},
      eprint={2204.05999},
      archivePrefix={arXiv},
      primaryClass={cs.SE}
}

@misc{zheng2024llamafactory,
      title={LlamaFactory: Unified Efficient Fine-Tuning of 100+ Language Models}, 
      author={Yaowei Zheng and Richong Zhang and Junhao Zhang and Yanhan Ye and Zheyan Luo and Yongqiang Ma},
      year={2024},
      eprint={2403.13372},
      archivePrefix={arXiv},
      primaryClass={cs.CL}
}

@article{Dagdelen2024,
  title = {Structured information extraction from scientific text with large language models},
  author = {Dagdelen, John and Dunn, Alexander and Lee, Sanghoon and Walker, Nicholas and Rosen, Andrew S. and Ceder, Gerbrand and Persson, Kristin A. and Jain, Anubhav},
  journal = {Nature Communications},
  volume = {15},
  number = {1},
  pages = {1418},
  year = {2024},
  doi = {10.1038/s41467-024-45563-x},
  issn = {2041-1723},
  url = {https://doi.org/10.1038/s41467-024-45563-x},
}

@article{Bzdok2024,
  title = {Data science opportunities of large language models for neuroscience and biomedicine},
  author = {Bzdok, Danilo and Thieme, Andrew and Levkovskyy, Oleksiy and Wren, Paul and Ray, Thomas and Reddy, Siva},
  journal = {Neuron},
  volume = {112},
  number = {5},
  pages = {698-717},
  year = {2024},
  month = {Mar},
  day = {6},
  doi = {10.1016/j.neuron.2024.01.016},
  issn = {1097-4199},
  pmid = {38340718},
  url = {https://doi.org/10.1016/j.neuron.2024.01.016},
}

@misc{tan2024large,
      title={Large Language Models for Data Annotation: A Survey}, 
      author={Zhen Tan and Alimohammad Beigi and Song Wang and Ruocheng Guo and Amrita Bhattacharjee and Bohan Jiang and Mansooreh Karami and Jundong Li and Lu Cheng and Huan Liu},
      year={2024},
      eprint={2402.13446},
      archivePrefix={arXiv},
      primaryClass={cs.CL}
}

@inproceedings{jTrans2022wang,
author = {Wang, Hao and Qu, Wenjie and Katz, Gilad and Zhu, Wenyu and Gao, Zeyu and Qiu, Han and Zhuge, Jianwei and Zhang, Chao},
title = {jTrans: jump-aware transformer for binary code similarity detection},
year = {2022},
isbn = {9781450393799},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/3533767.3534367},
doi = {10.1145/3533767.3534367},
booktitle = {Proceedings of the 31st ACM SIGSOFT International Symposium on Software Testing and Analysis},
pages = {1–13},
numpages = {13},
keywords = {Similarity Detection, Neural Networks, Datasets, Binary Analysis},
location = {<conf-loc>, <city>Virtual</city>, <country>South Korea</country>, </conf-loc>},
series = {ISSTA 2022}
}

@inproceedings{PalmTree21li,
author = {Li, Xuezixiang and Qu, Yu and Yin, Heng},
title = {PalmTree: Learning an Assembly Language Model for Instruction Embedding},
year = {2021},
isbn = {9781450384544},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/3460120.3484587},
doi = {10.1145/3460120.3484587},
booktitle = {Proceedings of the 2021 ACM SIGSAC Conference on Computer and Communications Security},
pages = {3236–3251},
numpages = {16},
keywords = {representation learning, language model, deep learning, binary analysis},
location = {Virtual Event, Republic of Korea},
series = {CCS '21}
}

@misc{hu2021lora,
      title={LoRA: Low-Rank Adaptation of Large Language Models}, 
      author={Edward J. Hu and Yelong Shen and Phillip Wallis and Zeyuan Allen-Zhu and Yuanzhi Li and Shean Wang and Lu Wang and Weizhu Chen},
      year={2021},
      eprint={2106.09685},
      archivePrefix={arXiv},
      primaryClass={cs.CL}
}

@misc{chen2023unleashing,
      title={Unleashing the potential of prompt engineering in Large Language Models: a comprehensive review}, 
      author={Banghao Chen and Zhaofeng Zhang and Nicolas Langrené and Shengxin Zhu},
      year={2023},
      eprint={2310.14735},
      archivePrefix={arXiv},
      primaryClass={cs.CL}
}

@misc{kong2024better,
      title={Better Zero-Shot Reasoning with Role-Play Prompting}, 
      author={Aobo Kong and Shiwan Zhao and Hao Chen and Qicheng Li and Yong Qin and Ruiqi Sun and Xin Zhou and Enzhi Wang and Xiaohang Dong},
      year={2024},
      eprint={2308.07702},
      archivePrefix={arXiv},
      primaryClass={cs.CL}
}

@misc{hou2023large,
    title={Large Language Models for Software Engineering: A Systematic Literature Review},
    author={Xinyi Hou and Yanjie Zhao and Yue Liu and Zhou Yang and Kailong Wang and Li Li and Xiapu Luo and David Lo and John Grundy and Haoyu Wang},
    year={2023},
    eprint={2308.10620},
    archivePrefix={arXiv},
    primaryClass={cs.SE}
}
